Real particle geodesics and thermodynamics of a black hole in Regular Schwarzschild-Anti de Sitter space-time

Regular Schwarzschild Anti-de-Sitter (RSch-AdS) spacetime, which is a maximally symmetric and Lorentzian manifold of negative curvature, is a solution of Einstein's field equations with a negative cosmological constant and a matter source with a Gaussian distribution. Studying of black hole (BH) in such a spacetime, known as RSch-AdS black hole, can be instructive from various aspects and lead to a better understanding of them. In this regard, geodesics of real particles around RSch-AdS black holes and RSch-AdS thermodynamics of BH are two important issues that we are going to evaluate in this research. For this purpose, we first obtain the geodesics of real particles based on the changes in the values of effective parameters such as mass distribution, angular momentum and cosmological constant numerically according to boundary conditions and interpret their behavior. Second, using the laws of thermodynamics, some aspects of BH, defined in this spacetime, such as temperature, entropy, heat capacity and Gibbs free energy are studied and discussed

==> article_aux <==
\relax 
\providecommand\hyper@newdestlabel[2]{}
\providecommand\HyperFirstAtBeginDocument{\AtBeginDocument}
\HyperFirstAtBeginDocument{\ifx\hyper@anchor\@undefined
\global\let\oldnewlabel\newlabel
\gdef\newlabel#1#2{\newlabelxx{#1}#2}
\gdef\newlabelxx#1#2#3#4#5#6{\oldnewlabel{#1}{{#2}{#3}}}
\AtEndDocument{\ifx\hyper@anchor\@undefined
\let\newlabel\oldnewlabel
\fi}
\fi}
\global\let\hyper@last\relax 
\gdef\HyperFirstAtBeginDocument#1{#1}
\providecommand\HyField@AuxAddToFields[1]{}
\providecommand\HyField@AuxAddToCoFields[2]{}
\citation{key-1}
\citation{key-2}
\citation{key-3}
\citation{key-4}
\@writefile{toc}{\contentsline {section}{\numberline {1}Introduction}{1}{section.1}\protected@file@percent }
\newlabel{sec:1}{{1}{1}{Introduction}{section.1}{}}
\citation{key-5,key-6}
\citation{key-7}
\citation{key-3}
\citation{key-7}
\citation{key-3}
\citation{key-8,key-9}
\citation{key-6,key-10}
\citation{key-10}
\citation{key-7,key-10}
\citation{key-11}
\citation{key-11}
\@writefile{toc}{\contentsline {section}{\numberline {2}RSch-AdS mathematical background}{3}{section.2}\protected@file@percent }
\newlabel{sec:2}{{2}{3}{RSch-AdS mathematical background}{section.2}{}}
\newlabel{equ1}{{1}{3}{RSch-AdS mathematical background}{equation.2.1}{}}
\newlabel{equ2}{{2}{3}{RSch-AdS mathematical background}{equation.2.2}{}}
\citation{key-12}
\citation{key-13}
\@writefile{lof}{\contentsline {figure}{\numberline {1}{\ignorespaces Mass density expressed in Equ. (\ref {equ2}), in which is distributed throughout a region with a linear size $\sqrt  {\theta }$ instead of being perfectly localized in a point due to uncertainty encoded in the coordinate space-time commutator. For $r\geq 8$ mass distribution is almost equal to zero.}}{4}{figure.caption.1}\protected@file@percent }
\providecommand*\caption@xref[2]{\@setref\relax\@undefined{#1}}
\newlabel{Fig1}{{1}{4}{Mass density expressed in Equ. (\ref {equ2}), in which is distributed throughout a region with a linear size $\sqrt {\theta }$ instead of being perfectly localized in a point due to uncertainty encoded in the coordinate space-time commutator. For $r\geq 8$ mass distribution is almost equal to zero}{figure.caption.1}{}}
\newlabel{equ3}{{3}{4}{RSch-AdS mathematical background}{equation.2.3}{}}
\newlabel{equ4}{{4}{4}{RSch-AdS mathematical background}{equation.2.4}{}}
\newlabel{equ5}{{5}{4}{RSch-AdS mathematical background}{equation.2.5}{}}
\@writefile{lof}{\contentsline {figure}{\numberline {2}{\ignorespaces Time metric function, $g_{tt}$, for RSch-AdS space-time vs radial distance $r$ for $M=0.5\sqrt  {\pi }$ and different values of cosmological constant (a) and for $\Lambda =-0.01$, and different values of mass i.e., $M=0.5\sqrt  {\pi }, \sqrt  {\pi }\hskip 1em\relax \text  {and}\hskip 1em\relax 1.5\sqrt  {\pi }$ (b).}}{5}{figure.caption.2}\protected@file@percent }
\newlabel{Fig2}{{2}{5}{Time metric function, $g_{tt}$, for RSch-AdS space-time vs radial distance $r$ for $M=0.5\sqrt {\pi }$ and different values of cosmological constant (a) and for $\Lambda =-0.01$, and different values of mass i.e., $M=0.5\sqrt {\pi }, \sqrt {\pi }\quad \text {and}\quad 1.5\sqrt {\pi }$ (b)}{figure.caption.2}{}}
\@writefile{lof}{\contentsline {subfigure}{\numberline{(a)}{\ignorespaces {}}}{5}{subfigure.2.1}\protected@file@percent }
\@writefile{lof}{\contentsline {subfigure}{\numberline{(b)}{\ignorespaces {}}}{5}{subfigure.2.2}\protected@file@percent }
\@writefile{lof}{\contentsline {figure}{\numberline {3}{\ignorespaces Time metric function, $g_{tt}$, for Sch-AdS space-time vs radial distance $r$ for a fixed mass, for example $M=\sqrt  {\pi }$, and different values of $\Lambda =-0.001,-0.01\hskip 1em\relax \text  {and} -0.1$ (a) and for a fixed $\Lambda =-0.01$ and $M=0.5\sqrt  {\pi },\sqrt  {\pi }\hskip 1em\relax \text  {and}\hskip 1em\relax 1.5\sqrt  {\pi }$ (b).}}{5}{figure.caption.3}\protected@file@percent }
\newlabel{Fig3}{{3}{5}{Time metric function, $g_{tt}$, for Sch-AdS space-time vs radial distance $r$ for a fixed mass, for example $M=\sqrt {\pi }$, and different values of $\Lambda =-0.001,-0.01\quad \text {and} -0.1$ (a) and for a fixed $\Lambda =-0.01$ and $M=0.5\sqrt {\pi },\sqrt {\pi }\quad \text {and}\quad 1.5\sqrt {\pi }$ (b)}{figure.caption.3}{}}
\@writefile{lof}{\contentsline {subfigure}{\numberline{(a)}{\ignorespaces {}}}{5}{subfigure.3.1}\protected@file@percent }
\@writefile{lof}{\contentsline {subfigure}{\numberline{(b)}{\ignorespaces {}}}{5}{subfigure.3.2}\protected@file@percent }
\newlabel{equ6}{{6}{5}{RSch-AdS mathematical background}{equation.2.6}{}}
\citation{key-14,key-15}
\citation{key-16}
\@writefile{toc}{\contentsline {section}{\numberline {3}Geodesics}{6}{section.3}\protected@file@percent }
\newlabel{sec:3}{{3}{6}{Geodesics}{section.3}{}}
\@writefile{toc}{\contentsline {subsection}{\numberline {3.1}Effective potential energy}{6}{subsection.3.1}\protected@file@percent }
\newlabel{subsec:3-1}{{3.1}{6}{Effective potential energy}{subsection.3.1}{}}
\newlabel{equ7}{{7}{6}{Effective potential energy}{equation.3.7}{}}
\newlabel{equ8}{{8}{6}{Effective potential energy}{equation.3.8}{}}
\@writefile{lof}{\contentsline {figure}{\numberline {4}{\ignorespaces Effective potential vs $r$ for $L=1$, $M=0.5\sqrt  {\pi }$, $\Lambda =-0.001$ (a) and previous values but $\Lambda =-0.01$ (b). Effective potential vs $r$ for $L=0.5$, $M=1.5\sqrt  {\pi }$, $\Lambda =-0.001$ (c) and previous values but $\Lambda =-0.01$ (d).}}{7}{figure.caption.4}\protected@file@percent }
\newlabel{Fig4}{{4}{7}{Effective potential vs $r$ for $L=1$, $M=0.5\sqrt {\pi }$, $\Lambda =-0.001$ (a) and previous values but $\Lambda =-0.01$ (b). Effective potential vs $r$ for $L=0.5$, $M=1.5\sqrt {\pi }$, $\Lambda =-0.001$ (c) and previous values but $\Lambda =-0.01$ (d)}{figure.caption.4}{}}
\@writefile{lof}{\contentsline {subfigure}{\numberline{(a)}{\ignorespaces {}}}{7}{subfigure.4.1}\protected@file@percent }
\@writefile{lof}{\contentsline {subfigure}{\numberline{(b)}{\ignorespaces {}}}{7}{subfigure.4.2}\protected@file@percent }
\@writefile{lof}{\contentsline {subfigure}{\numberline{(c)}{\ignorespaces {}}}{7}{subfigure.4.3}\protected@file@percent }
\@writefile{lof}{\contentsline {subfigure}{\numberline{(d)}{\ignorespaces {}}}{7}{subfigure.4.4}\protected@file@percent }
\@writefile{toc}{\contentsline {subsection}{\numberline {3.2}Geodesics equations for RSch-AdS space-time}{8}{subsection.3.2}\protected@file@percent }
\newlabel{subsec:3-2}{{3.2}{8}{Geodesics equations for RSch-AdS space-time}{subsection.3.2}{}}
\newlabel{equ9}{{9}{8}{Geodesics equations for RSch-AdS space-time}{equation.3.9}{}}
\newlabel{equ10}{{10}{8}{Geodesics equations for RSch-AdS space-time}{equation.3.10}{}}
\newlabel{equ11}{{11}{8}{Geodesics equations for RSch-AdS space-time}{equation.3.11}{}}
\newlabel{equ12}{{12}{8}{Geodesics equations for RSch-AdS space-time}{equation.3.12}{}}
\citation{key-15,key-17,key-18,key-19}
\@writefile{lof}{\contentsline {figure}{\numberline {5}{\ignorespaces Particle trajectory plotted for $M=0.5\sqrt  {\pi }$, $L=1$, $\Lambda =-0.001$, $\dot  {r}_{0}(\tau )=0$, $r_{0}(\tau )=15$ and $\tau =[0,100000]$ as initial conditions (a). Reiteration the previous process but this time for $\Lambda =-0.01$ and $r_{0}(0)=16.5$ and $\tau =[0,10000]$.}}{9}{figure.caption.5}\protected@file@percent }
\newlabel{Fig5}{{5}{9}{Particle trajectory plotted for $M=0.5\sqrt {\pi }$, $L=1$, $\Lambda =-0.001$, $\dot {r}_{0}(\tau )=0$, $r_{0}(\tau )=15$ and $\tau =[0,100000]$ as initial conditions (a). Reiteration the previous process but this time for $\Lambda =-0.01$ and $r_{0}(0)=16.5$ and $\tau =[0,10000]$}{figure.caption.5}{}}
\@writefile{lof}{\contentsline {subfigure}{\numberline{(a)}{\ignorespaces {}}}{9}{subfigure.5.1}\protected@file@percent }
\@writefile{lof}{\contentsline {subfigure}{\numberline{(b)}{\ignorespaces {}}}{9}{subfigure.5.2}\protected@file@percent }
\@writefile{toc}{\contentsline {subsection}{\numberline {3.3}initial conditions}{9}{subsection.3.3}\protected@file@percent }
\newlabel{subsec:3-3}{{3.3}{9}{initial conditions}{subsection.3.3}{}}
\citation{key-20}
\citation{key-10,key-21}
\@writefile{lof}{\contentsline {figure}{\numberline {6}{\ignorespaces Particle trajectory plotted for $M=1.5\sqrt  {\pi }$, $L=0.5$, $\Lambda =-0.001$, $\dot  {r}_{0}(\tau )=0$, $r_{0}(\tau )=10$ and $\tau =[0,11000]$ as initial conditions (a). Reiteration the previous process, but this time for $\Lambda =-0.01$, $r_{0}=13.5$ and $\tau =[0,5000]$.}}{11}{figure.caption.6}\protected@file@percent }
\newlabel{Fig6}{{6}{11}{Particle trajectory plotted for $M=1.5\sqrt {\pi }$, $L=0.5$, $\Lambda =-0.001$, $\dot {r}_{0}(\tau )=0$, $r_{0}(\tau )=10$ and $\tau =[0,11000]$ as initial conditions (a). Reiteration the previous process, but this time for $\Lambda =-0.01$, $r_{0}=13.5$ and $\tau =[0,5000]$}{figure.caption.6}{}}
\@writefile{lof}{\contentsline {subfigure}{\numberline{(a)}{\ignorespaces {}}}{11}{subfigure.6.1}\protected@file@percent }
\@writefile{lof}{\contentsline {subfigure}{\numberline{(b)}{\ignorespaces {}}}{11}{subfigure.6.2}\protected@file@percent }
\@writefile{toc}{\contentsline {section}{\numberline {4}Thermodynamics of RSch-AdS }{11}{section.4}\protected@file@percent }
\newlabel{sec:4}{{4}{11}{Thermodynamics of RSch-AdS}{section.4}{}}
\citation{key-11,key-22}
\citation{key-23}
\@writefile{lof}{\contentsline {figure}{\numberline {7}{\ignorespaces For all attributed values of mass and $r\leq 3.55$, the tangential pressure is negative and then becomes a little positive but quickly approaches to zero. }}{12}{figure.caption.7}\protected@file@percent }
\newlabel{Fig7}{{7}{12}{For all attributed values of mass and $r\leq 3.55$, the tangential pressure is negative and then becomes a little positive but quickly approaches to zero}{figure.caption.7}{}}
\newlabel{equ13}{{13}{12}{Thermodynamics of RSch-AdS}{equation.4.13}{}}
\newlabel{equ14}{{14}{12}{Thermodynamics of RSch-AdS}{equation.4.14}{}}
\newlabel{equ15}{{15}{13}{Thermodynamics of RSch-AdS}{equation.4.15}{}}
\newlabel{equ16}{{16}{13}{Thermodynamics of RSch-AdS}{equation.4.16}{}}
\@writefile{lof}{\contentsline {figure}{\numberline {8}{\ignorespaces Mass of RSch-AdS-BH in terms of radius (a) vs mass of AdS-BH in terms of radius (b) for different values of $\Lambda $.}}{13}{figure.caption.8}\protected@file@percent }
\newlabel{Fig8}{{8}{13}{Mass of RSch-AdS-BH in terms of radius (a) vs mass of AdS-BH in terms of radius (b) for different values of $\Lambda $}{figure.caption.8}{}}
\@writefile{lof}{\contentsline {subfigure}{\numberline{(a)}{\ignorespaces {}}}{13}{subfigure.8.1}\protected@file@percent }
\@writefile{lof}{\contentsline {subfigure}{\numberline{(b)}{\ignorespaces {}}}{13}{subfigure.8.2}\protected@file@percent }
\citation{key-24}
\@writefile{lof}{\contentsline {figure}{\numberline {9}{\ignorespaces Mass of RSch-AdS-BH in terms of entropy (a) vs mass of AdS-BH in terms of entropy (b) for different values of $\Lambda $.}}{14}{figure.caption.9}\protected@file@percent }
\newlabel{Fig9}{{9}{14}{Mass of RSch-AdS-BH in terms of entropy (a) vs mass of AdS-BH in terms of entropy (b) for different values of $\Lambda $}{figure.caption.9}{}}
\@writefile{lof}{\contentsline {subfigure}{\numberline{(a)}{\ignorespaces {}}}{14}{subfigure.9.1}\protected@file@percent }
\@writefile{lof}{\contentsline {subfigure}{\numberline{(b)}{\ignorespaces {}}}{14}{subfigure.9.2}\protected@file@percent }
\newlabel{equ17}{{17}{14}{Thermodynamics of RSch-AdS}{equation.4.17}{}}
\newlabel{equ18}{{18}{14}{Thermodynamics of RSch-AdS}{equation.4.18}{}}
\@writefile{lof}{\contentsline {figure}{\numberline {10}{\ignorespaces Black hole event horizon temperature for different values of $\Lambda $ in terms of $r_{\text  {H}}$, (a) for RSch-AdS case and (b) for AdS one.}}{15}{figure.caption.10}\protected@file@percent }
\newlabel{Fig10}{{10}{15}{Black hole event horizon temperature for different values of $\Lambda $ in terms of $r_{\text {H}}$, (a) for RSch-AdS case and (b) for AdS one}{figure.caption.10}{}}
\@writefile{lof}{\contentsline {subfigure}{\numberline{(a)}{\ignorespaces {}}}{15}{subfigure.10.1}\protected@file@percent }
\@writefile{lof}{\contentsline {subfigure}{\numberline{(b)}{\ignorespaces {}}}{15}{subfigure.10.2}\protected@file@percent }
\newlabel{equ19}{{19}{15}{Thermodynamics of RSch-AdS}{equation.4.19}{}}
\newlabel{equ20}{{20}{15}{Thermodynamics of RSch-AdS}{equation.4.20}{}}
\newlabel{equ21}{{21}{15}{Thermodynamics of RSch-AdS}{equation.4.21}{}}
\@writefile{lof}{\contentsline {figure}{\numberline {11}{\ignorespaces Black hole event horizon temperature for different values of $\Lambda $ in terms of $S$, for RSch-AdS case (a) and for AdS one (b).}}{16}{figure.caption.11}\protected@file@percent }
\newlabel{Fig11}{{11}{16}{Black hole event horizon temperature for different values of $\Lambda $ in terms of $S$, for RSch-AdS case (a) and for AdS one (b)}{figure.caption.11}{}}
\@writefile{lof}{\contentsline {subfigure}{\numberline{(a)}{\ignorespaces {}}}{16}{subfigure.11.1}\protected@file@percent }
\@writefile{lof}{\contentsline {subfigure}{\numberline{(b)}{\ignorespaces {}}}{16}{subfigure.11.2}\protected@file@percent }
\newlabel{equ22}{{22}{16}{Thermodynamics of RSch-AdS}{equation.4.22}{}}
\newlabel{equ23}{{23}{16}{Thermodynamics of RSch-AdS}{equation.4.23}{}}
\newlabel{equ24}{{24}{17}{Thermodynamics of RSch-AdS}{equation.4.24}{}}
\@writefile{lof}{\contentsline {figure}{\numberline {12}{\ignorespaces Heat capacity in terms of entropy for different values of $\Lambda $, for RSch-AdS black hole (a) and AdS-black hole (b) . }}{17}{figure.caption.12}\protected@file@percent }
\newlabel{Fig12}{{12}{17}{Heat capacity in terms of entropy for different values of $\Lambda $, for RSch-AdS black hole (a) and AdS-black hole (b) }{figure.caption.12}{}}
\@writefile{lof}{\contentsline {subfigure}{\numberline{(a)}{\ignorespaces {}}}{17}{subfigure.12.1}\protected@file@percent }
\@writefile{lof}{\contentsline {subfigure}{\numberline{(b)}{\ignorespaces {}}}{17}{subfigure.12.2}\protected@file@percent }
\newlabel{equ25}{{25}{17}{Thermodynamics of RSch-AdS}{equation.4.25}{}}
\newlabel{equ26}{{26}{17}{Thermodynamics of RSch-AdS}{equation.4.26}{}}
\newlabel{equ27}{{27}{18}{Thermodynamics of RSch-AdS}{equation.4.27}{}}
\@writefile{lof}{\contentsline {figure}{\numberline {13}{\ignorespaces Gibs free energy in terms of entropy for different values of $\Lambda $, for RSch-AdS black hole (a) and AdS-black hole (b) . }}{18}{figure.caption.13}\protected@file@percent }
\newlabel{Fig13}{{13}{18}{Gibs free energy in terms of entropy for different values of $\Lambda $, for RSch-AdS black hole (a) and AdS-black hole (b) }{figure.caption.13}{}}
\@writefile{lof}{\contentsline {subfigure}{\numberline{(a)}{\ignorespaces {}}}{18}{subfigure.13.1}\protected@file@percent }
\@writefile{lof}{\contentsline {subfigure}{\numberline{(b)}{\ignorespaces {}}}{18}{subfigure.13.2}\protected@file@percent }
\@writefile{toc}{\contentsline {section}{\numberline {5}Conclusion}{19}{section.5}\protected@file@percent }
\newlabel{sec:5}{{5}{19}{Conclusion}{section.5}{}}
\bibcite{key-1}{{1}{}{{}}{{}}}
\bibcite{key-2}{{2}{}{{}}{{}}}
\bibcite{key-3}{{3}{}{{}}{{}}}
\bibcite{key-4}{{4}{}{{}}{{}}}
\bibcite{key-5}{{5}{}{{}}{{}}}
\bibcite{key-6}{{6}{}{{}}{{}}}
\bibcite{key-7}{{7}{}{{}}{{}}}
\bibcite{key-8}{{8}{}{{}}{{}}}
\bibcite{key-9}{{9}{}{{}}{{}}}
\bibcite{key-10}{{10}{}{{}}{{}}}
\bibcite{key-11}{{11}{}{{}}{{}}}
\bibcite{key-12}{{12}{}{{}}{{}}}
\bibcite{key-13}{{13}{}{{}}{{}}}
\bibcite{key-14}{{14}{}{{}}{{}}}
\bibcite{key-15}{{15}{}{{}}{{}}}
\bibcite{key-16}{{16}{}{{}}{{}}}
\bibcite{key-17}{{17}{}{{}}{{}}}
\bibcite{key-18}{{18}{}{{}}{{}}}
\bibcite{key-19}{{19}{}{{}}{{}}}
\bibcite{key-20}{{20}{}{{}}{{}}}
\bibcite{key-21}{{21}{}{{}}{{}}}
\bibcite{key-22}{{22}{}{{}}{{}}}
\bibcite{key-23}{{23}{}{{}}{{}}}
\bibcite{key-24}{{24}{}{{}}{{}}}
\providecommand\NAT@force@numbers{}\NAT@force@numbers
\gdef \@abspage@last{22}


==> article_out <==
\BOOKMARK [1][-]{section.1}{\376\377\000I\000n\000t\000r\000o\000d\000u\000c\000t\000i\000o\000n}{}% 1
\BOOKMARK [1][-]{section.2}{\376\377\000R\000S\000c\000h\000-\000A\000d\000S\000\040\000m\000a\000t\000h\000e\000m\000a\000t\000i\000c\000a\000l\000\040\000b\000a\000c\000k\000g\000r\000o\000u\000n\000d}{}% 2
\BOOKMARK [1][-]{section.3}{\376\377\000G\000e\000o\000d\000e\000s\000i\000c\000s}{}% 3
\BOOKMARK [2][-]{subsection.3.1}{\376\377\000E\000f\000f\000e\000c\000t\000i\000v\000e\000\040\000p\000o\000t\000e\000n\000t\000i\000a\000l\000\040\000e\000n\000e\000r\000g\000y}{section.3}% 4
\BOOKMARK [2][-]{subsection.3.2}{\376\377\000G\000e\000o\000d\000e\000s\000i\000c\000s\000\040\000e\000q\000u\000a\000t\000i\000o\000n\000s\000\040\000f\000o\000r\000\040\000R\000S\000c\000h\000-\000A\000d\000S\000\040\000s\000p\000a\000c\000e\000-\000t\000i\000m\000e}{section.3}% 5
\BOOKMARK [2][-]{subsection.3.3}{\376\377\000i\000n\000i\000t\000i\000a\000l\000\040\000c\000o\000n\000d\000i\000t\000i\000o\000n\000s}{section.3}% 6
\BOOKMARK [1][-]{section.4}{\376\377\000T\000h\000e\000r\000m\000o\000d\000y\000n\000a\000m\000i\000c\000s\000\040\000o\000f\000\040\000R\000S\000c\000h\000-\000A\000d\000S\000\040}{}% 7
\BOOKMARK [1][-]{section.5}{\376\377\000C\000o\000n\000c\000l\000u\000s\000i\000o\000n}{}% 8

